Tutel: Adaptive Mixture-of-Experts at Scale

Sparsely-gated mixture-of-experts (MoE) has been widely adopted to scale deep learning models to trillion-plus parameters with fixed computational cost. The algorithmic performance of MoE relies on its token routing mechanism that forwards each input token to the right sub-models or experts. While token routing dynamically determines the amount of expert workload at runtime, existing systems suffer inefficient computation due to their static execution, namely static parallelism and pipelining, which does not adapt to the dynamic workload. We present Flex, a highly scalable stack design and implementation for MoE with dynamically adaptive parallelism and pipelining. Flex designs an identical layout for distributing MoE model parameters and input data, which can be leveraged by all possible parallelism or pipelining methods without any mathematical inequivalence or tensor migration overhead. This enables adaptive parallelism/pipelining optimization at zero cost during runtime. Based on this key design, Flex also implements various MoE acceleration techniques. Aggregating all techniques, Flex finally delivers huge speedup at any scale -- 4.96x and 5.75x speedup of a single MoE layer over 16 and 2,048 A100 GPUs, respectively, over the previous state-of-the-art. Our evaluation shows that Flex efficiently and effectively runs a real-world MoE-based model named SwinV2-MoE, built upon Swin Transformer V2, a state-of-the-art computer vision architecture. On efficiency, Flex accelerates SwinV2-MoE, achieving up to 1.55x and 2.11x speedup in training and inference over Fairseq, respectively. On effectiveness, the SwinV2-MoE model achieves superior accuracy in both pre-training and down-stream computer vision tasks such as COCO object detection than the counterpart dense model, indicating the readiness of Flex for end-to-end real-world model training and inference.

==> sections/6Related.tex <==
\section{Related Work}

\paragraph{MoE Frameworks.}
% Fairseq MoE~\cite{fairseq}, Deepspeed MoE~\cite{deepspeed-moe}, and FastMoE/FasterMoE~\cite{he2022fastermoe} are three popular GPU-based MoE frameworks. Fairseq MoE and Deepspeed MoE leverage the same MoE computation method as GShard~\cite{gshard} and both achieve similar poor performance at a large scale. FastMoE/FasterMoE~\cite{he2022fastermoe} proposes different gating algorithms, which are not computationally equivalent with GShard. Furthermore, proposed ``Shadow Expert'' and ``Smart Schedule'' in FasterMoE have several adaption restrictions on dataset, expert portage cost, and memory for caching. \tutel{} keeps the same computation logic as GShard to ensure algorithmic correctness (shown in~\cref{ssec:eval-swin-moe}) and achieves deterministic gain on typical environments and hyper-parameter settings, which adapts MoE frameworks to exa-scale without harming algorithmic results.
While GShard~\cite{gshard} provides a computation logic that ensures algorithmic correctness of MoE, several popular MoE frameworks~\cite{fairseq,deepspeed-moe} follow the same logic but perform poorly at a large scale. FastMoE/FaterMoE~\cite{he2022fastermoe} proposes different gating algorithms that are not computationally equivalent with GShard. Furthermore, proposed \textit{shadow expert} and \textit{smart schedule} in FasterMoE introduce several restrictions on dataset, expert portage cost, and memory for caching. \tutel{} keeps the same computation logic as GShard and achieves deterministic gain on typical environments and hyper-parameter settings, which adapts MoE frameworks to exa-scale without harming algorithmic results.

\iffalse
\paragraph{\AtoA{} Collective Communication.}

NCCL is the state-of-the-art collective communication library on NVIDIA GPUs and InfiniBand, while there is also a forked version, RCCL~\cite{rccl}, on AMD GPUs that shares similar implementations.
% NCCL recently released 2.12 version that introduces a new feature called \textit{PXN}~\cite{pxn}, which avoids cross-rail communication by moving the sender GPU's data to another local GPU in the server that belongs to the same rail with the remote receiver GPU before pushing the data to the InfiniBand network. PXN shared a similar idea with 2DH \AtoA{} and would deliver gain comparing to NCCL's original \AtoA{}, but 
The recent NCCL 2.12 version introduces a feature called \textit{PXN}~\cite{pxn} that avoids cross-rail communication by leveraging intra-node communication. While PXN delivers a similar gain as 2DH \AtoA{} in terms of intra-node chunk aggregation,
it still does not address the challenge of small message merging overhead in~\cref{ssec:2dha2a}.
% , that is, it would use NVLink to transfer many small chunks and incur increasing latency when scaling out.
PXN claims $\sim2.5\times$ speedup for 1 MiB size at 1,024 GPUs~\cite{pxn}, while our algorithm shows ten to twenty times of speedup for the same size at 1,024 or 2,048 GPUs.
% NCCL's results showed PXN has $\sim 2.5$ times speedup for 1 MiB size on 1024-GPU~\cite{pxn}, while our algorithm had ten to twenty times speedup for the same size on 1024 or 2048 GPUs.
Please note that PXN is a parallel work with this work, and it is yet early to deliver an extensive comparison in this paper.
\fi

